On a unit ball placement problem: covering the most points in fixed dimension

For $N$ distinct sites in fixed dimension $D\ge 2$, we give a deterministic algorithm that places a closed unit ball covering the most sites. It returns the centre, count and all covered indices in $O_D(N^D)$ time and $O_D(N)$ extra words on an exact real random-access machine. The same bounds hold for maximizing the sum of nonnegative weights of covered sites. For $D\ge 3$, we search two-spheres of possible centres determined by $D-2$ sites on the ball boundary. Each site gives a cap of centres whose ball covers it. To find a point where the covering caps have maximum total weight, we use stereographic projection and at most two planar searches over weighted closed disks and their closed exteriors. For $m$ circles of arbitrary positive radii, each planar search takes $O(m^2)$ time and $O(m)$ extra words. A linear-time reduction shows that any fixed saving in the exponent $D$ for deterministic placement would carry over to deciding whether $D+1$ of $N$ distinct integer points lie on a common hyperplane.

==> figures/ball-depth/cover-vectors.tex <==
\coordinate (cover1) at (0.24253563,-0.58300837);
\coordinate (cover2) at (0.53357838,0.20405293);
\coordinate (cover3) at (-0.63059263,0.02915042);
\coordinate (cover4) at (0.06063391,0.45371216);
\coordinate (cover5) at (0.06063391,-0.74521634);


==> figures/cell-colours.tex <==
% Selected cell-family palette, exact sRGB.
\definecolor{cellW}{HTML}{FFFFFF}%
\definecolor{cellL}{HTML}{FFFFFF}%
\definecolor{cellR}{HTML}{FFFFFF}%
\definecolor{cellR1}{HTML}{FFFFFF}%
\definecolor{cellR2}{HTML}{FFFFFF}%
\definecolor{cellR3}{HTML}{FFFFFF}%
\definecolor{cellR4}{HTML}{FFFFFF}%
\definecolor{cellB}{HTML}{F5E4A0}%
\definecolor{cellI}{HTML}{9BCFBE}%
\definecolor{cellT}{HTML}{B5C5E7}%
\definecolor{cellT1}{HTML}{9CAED9}%
\definecolor{cellT2}{HTML}{D7E3F3}%
\definecolor{cellT3}{HTML}{788CC2}%
\definecolor{cellT4}{HTML}{EAF1FA}%
\definecolor{cellT5}{HTML}{B0C0E0}%
\definecolor{cellT6}{HTML}{C2D2EA}%
\definecolor{cellT7}{HTML}{899CCE}%
\definecolor{cellI1}{HTML}{B5DECF}%
\definecolor{cellI2}{HTML}{DDF1E8}%
\definecolor{cellI3}{HTML}{70B3A1}%
\definecolor{cellI4}{HTML}{92C8B7}%
\input{figures/cell-hierarchy-paths}
\unskip%
\providecommand{\cellPaint}[1]{\csname cellPaint#1\endcsname}%
\providecommand{\cellNode}[1]{cell#1}%

